MoMa-Kitchen: A 100K+ Benchmark for Affordance-Grounded Last-Mile Navigation in Mobile Manipulation

In mobile manipulation, navigation and manipulation are often treated as separate problems, resulting in a significant gap between merely approaching an object and engaging with it effectively. Many navigation approaches primarily define success by proximity to the target, often overlooking the necessity for optimal positioning that facilitates subsequent manipulation. To address this, we introduce MoMa-Kitchen, a benchmark dataset comprising over 100k samples that provide training data for models to learn optimal final navigation positions for seamless transition to manipulation. Our dataset includes affordance-grounded floor labels collected from diverse kitchen environments, in which robotic mobile manipulators of different models attempt to grasp target objects amidst clutter. Using a fully automated pipeline, we simulate diverse real-world scenarios and generate affordance labels for optimal manipulation positions. Visual data are collected from RGB-D inputs captured by a first-person view camera mounted on the robotic arm, ensuring consistency in viewpoint during data collection. We also develop a lightweight baseline model, NavAff, for navigation affordance grounding that demonstrates promising performance on the MoMa-Kitchen benchmark. Our approach enables models to learn affordance-based final positioning that accommodates different arm types and platform heights, thereby paving the way for more robust and generalizable integration of navigation and manipulation in embodied AI. Project page: \href{https://momakitchen.github.io/}{https://momakitchen.github.io/}.

==> sec/4_analysis.tex <==
\section{Dataset Overview}
\label{sec:analysis}

\textcolor{red}{\{I suggest this section can be combined with Section 2, and for the Task Definition, add it at the begining of section 2, for the Dataset Statistics, add it at the end of Section 2 as a subsection titled "Generated Dataset Statistics."\}}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/arms_category_affor.pdf}
    \caption{\textbf{(a) Robot arms used in \ours.} The end-effectors of the Panda, Flexiv, and xArm6 robots are grippers, while the end-effector of the UR5e is a suction cup. 
    \textbf{(b) Object categories utilized in \ours.} Each category consists of multiple object instances. 
    Rigid and articulated objects serve as manipulation targets, while obstacle objects are strategically placed around the target to enhance scene complexity. 
    \textbf{(c) Examples of affordance maps in \ours.} Discrete affordance values are first collected (top) by moving the mobile manipulator and allowing it to interact with the target. 
    Gaussian interpolation is then applied to obtain a smooth affordance map (bottom).}
    \label{fig:arms_category_affor}
\end{figure*}


\textbf{Task Definition}.
\ours focuses on determining feasible final navigation positions that enable successful manipulation in cluttered environments. 
Given RGB-D inputs from a first-person camera and robot-specific parameters (e.g., arm reach, base height), the goal is to produce an affordance map over the floor. 
This map indicates where the robot can position itself to reliably manipulate the target while accounting for obstacles, bridging navigation and manipulation within a unified pipeline.

% The primary objective of \ours is to enable a mobile manipulator to determine optimal manipulation positions through affordance-aware planning in complex, cluttered environments. 
% Specifically, our system generates navigation affordance grounding maps that identify viable floor positions from which the mobile manipulator can successfully interact with target objects while avoiding environmental obstacles. 
% Given an RGB image $\mathbf{I}$ and its corresponding depth map $\mathbf{D}$ captured by the robot’s onboard camera, along with robot-specific information including base height and arm reach, our \ourmodel model generates precise affordance predictions on the floor for feasible manipulation positions. 
% By reformulating the navigation-to-manipulation problem as a visual grounding task through floor affordance mapping, our approach effectively bridges the gap between navigating planning and manipulation execution, thereby facilitating robust task completion in real-world scenarios. 


% \subsection{Dataset Statistics}
\begin{table}[t]
    \footnotesize
    \centering
    \caption{\textbf{Dataset Split Statistics}}
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{@{}lccc@{}}
            \toprule
            Split                & Scenes & Configurations & Episodes\\
            \midrule
            Train                & $456$ & $11,408$ & $102,687$ \\
            Test (Unseen Scenes) & $113$ & $2,747$ & $24,656$ \\
            \bottomrule
            \end{tabular}
    }
    
    \vspace{5pt}
    
    \label{tab:data_split}
    \vspace{-10pt}
\end{table}


\vspace{0.5em}
\noindent\textbf{Dataset Statistics}.
As summarized in Table~\ref{tab:data_split}, \ours spans 569 kitchen scenes, each with procedural variations in objects and obstacles. These configurations yield over 127k episodes, each capturing an RGB-D view and the resulting affordance map. 
Four robot arms (Flexiv, Panda, UR5e, xArm6) are deployed to ensure diverse reachability constraints and end-effector types. 
The dataset covers 14 kitchen-relevant categories (5 rigid, 5 articulated, and 4 obstacle types), providing a broad spectrum of layouts and manipulation targets.
During data collection, each configuration is labeled via discrete success/failure outcomes for different robot placements. 
These discrete labels are then interpolated to produce dense affordance maps (see Fig.~\ref{fig:arms_category_affor}(c)). 
Collectively, \ours provides large-scale supervision for end-to-end training of navigation-to-manipulation models that generalize across varying hardware and scene complexity.

% \noindent \textbf{Dataset Splits.} The composition of \ours is detailed in~\cref{tab:data_split}. 
% \ours encompasses $569$ distinct scenes, each with unique base furniture and layout. 
% For each scene, we generate approximately $25$ configurations, maintaining the core layout while varying the types and positions of obstacles and target objects. 
% Each configuration is then captured from approximately $10$ different camera viewpoints, ultimately yielding $127,343$ episodes.

% \noindent \textbf{Robot Arms}. As shown in~\cref{fig:arms_category_affor} (a), we employ diverse robotic platforms, including Flexiv, Panda, UR5e, and xArm6, to improve generalization. 
% These platforms feature different end-effectors: Panda, Flexiv, and xArm6 are equipped with parallel grippers, while UR5e utilizes a suction-based end-effector. 
% For each scene, we randomly select one of these robotic platforms for data collection.

% \noindent \textbf{Object Categories}. We present the object categories of \ours in~\cref{fig:arms_category_affor} (b). 
% Our dataset comprises $14$ common object categories specifically selected from kitchen environments. 
% Specifically, the dataset includes $5$ rigid object categories, $5$ articulated object categories, and $4$ obstacle categories. 
% In our setup, rigid categories are used for gripper manipulation tasks involving grasping and short-distance translations, while articulated categories are used for joint-based rotational operations. 
% The obstacle categories are strategically incorporated to enhance environmental complexity and diversity, creating more challenging and realistic interaction scenarios.

% \noindent \textbf{Affordance Ground Truth}. The navigation affordance ground truth map examples in \ours are shown in~\cref{fig:arms_category_affor} (c).
% For each configuration in \ours, we collect discrete success/failure values by moving the mobile robot and interacting with the target in the scene. 
% To obtain a more continuous map, we apply Gaussian interpolation to the collected data, resulting in the final navigation affordance map.

